Tile2Vec: Unsupervised representation learning for spatially distributed data

Geospatial analysis lacks methods like the word vector representations and pre-trained networks that significantly boost performance across a wide range of natural language and computer vision tasks. To fill this gap, we introduce Tile2Vec, an unsupervised representation learning algorithm that extends the distributional hypothesis from natural language -- words appearing in similar contexts tend to have similar meanings -- to spatially distributed data. We demonstrate empirically that Tile2Vec learns semantically meaningful representations on three datasets. Our learned representations significantly improve performance in downstream classification tasks and, similar to word vectors, visual analogies can be obtained via simple arithmetic in the latent space.

==> 01_fig_dg.tex <==
\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{figures/fig_dg.jpg}
  \caption{Digital Globe composites of (Left) Addis Ababa, Ethiopia and (Right) Modesto, California.}
  \label{fig:dg}
\end{figure}

==> 01_fig_loss.tex <==
\begin{figure}[H]
\centering
  \includegraphics[width=0.8\linewidth]{figures/fig_loss.png}
  \caption{Training loss and CDL accuracy per epoch over 10 trials. Note that the consistent decrease in the unsupervised training loss (left) leads to a corresponding increase in performance on the downstream task of interest (right). Each epoch represents 100k triplets; even after training for many epochs we don't observe any overfitting.}
  \label{fig:loss}
\end{figure}
